Insights into LSTM Fully Convolutional Networks for Time Series Classification

Long Short Term Memory Fully Convolutional Neural Networks (LSTM-FCN) and Attention LSTM-FCN (ALSTM-FCN) have shown to achieve state-of-the-art performance on the task of classifying time series signals on the old University of California-Riverside (UCR) time series repository. However, there has been no study on why LSTM-FCN and ALSTM-FCN perform well. In this paper, we perform a series of ablation tests (3627 experiments) on LSTM-FCN and ALSTM-FCN to provide a better understanding of the model and each of its sub-module. Results from the ablation tests on ALSTM-FCN and LSTM-FCN show that the LSTM and the FCN blocks perform better when applied in a conjoined manner. Two z-normalizing techniques, z-normalizing each sample independently and z-normalizing the whole dataset, are compared using a Wilcoxson signed-rank test to show a statistical difference in performance. In addition, we provide an understanding of the impact dimension shuffle has on LSTM-FCN by comparing its performance with LSTM-FCN when no dimension shuffle is applied. Finally, we demonstrate the performance of the LSTM-FCN when the LSTM block is replaced by a GRU, basic RNN, and Dense Block.

==> introduction-old.tex <==
Over the past decade, there has been an increased interest in time series classification and clustering. Time series data is ubiquitous, existing in weather readings, financial recordings, industrial observations, and psychological signals \cite{Wang_2017}. In this paper two deep learning models to classify time series datasets are proposed, both of which outperform existing state-of-the-art models.

Recently, deep learning approaches have been employed with time series classification algorithms. Multi-scale CNN (MCNN) \cite{cui2016multi}, fully convolutional network (FCN) \cite{wang2017time}, and residual network (ResNet) \cite{wang2017time} are deep learning approaches that take advantage of convolutional neural networks (CNN) for end-to-end classification of univariate time series. MCNN uses down-sampling, skip sampling and sliding window to preprocess the data. The classifier is highly dependent on the preprocessing and the large set of hyperparameters. On the other hand, FCN and ResNet do not require any heavy pre-processing on the data or feature crafting. In this paper, we improve the performance of FCN by concatenating CNN with a Long Term Short Term (LSTM) layer, LSTMFCN, or a LSTM layer with attention, ALSTMFCN. Similar to FCN, both proposed models can develop a Class Activation Maps (CAM) on the convolutional layers to detect regions that contribute to the class label more than others. In addition, the Attention LSTM layer can also be used detect regions that contribute to the class label through its VISUALS. Results indicate the new proposed models, LSTMFCN and ALSTMFCN, dramatically improve performance on the University of California Riverside (UCR) Benchmark datasets \cite{UCRArchive}.  

A plethora of research have been done using feature-based approaches or methods to extract a set of features that represent time series patterns. Bag-of-Words (BoW) \cite{Lin_2007}, Bag-of-features (TSBF) \cite{Baydogan_2013}, Bag-of-SFA-Symbols (BOSS) \cite{Sch_fer_2014}, BOSSVS \cite{schafer2016scalable}, Word ExtrAction for time SEries cLassification (WEASEL) \cite{Schafer_2017}, have obtained promising results in the field. Bag-of-words quantizes the extracted features and feeds the BoW into a classifier. TSBF extracts multiple subsequences of random local information, which a supervised learner condenses into a cookbook used to predict time series labels. BOSS introduces a combination of a distance based classifier and histograms. The histograms represent substructures of a time series that are created using a symbolic Fourier approximation. BOSSVS extends this method by proposing a vector space model to reduce time complexity while maintaining performance.  WEASEL converts time series into feature vectors using a sliding window. Machine learning algorithms utilize these feature vectors to detect and classify the time series.  All these classifiers require heavy feature extraction and feature crafting. One of the major advantages of LSTMFCN and ALSTMFCN is it does not require heavy preprocessing or feature crafting.

Ensemble algorithms also yield state-of-the-art performance with time series classification problems. Three of the most successful ensemble algorithms that integrate various features of a time series are Elastic Ensemble (PROP) \cite{Lines_2014}, a model that integrates 11 time series classifiers using a weighted ensemble method, Shapelet ensemble (SE) \cite{Bagnall_2016a}, a model that applies a heterogeneous ensemble onto transformed “shapelets”, and a flat collective of transform based ensembles (COTE) \cite{bagnall2015time}, a model that fuses 35 various classifiers into 1 classifier. LSTMFCN and ALSTMFCN produce better results than the Ensemble algorithms on a majority of the UCR Benchmark datasets. 

This paper proposes two deep learning models for end-to-end time series classification. The proposed models do not require heavy pre-processing on the data or feature crafting. Both the models are tested on all 85 UCR time series benchmarks and outperforms most of the state-of-the-art models. The remainder of the paper is organized as follows. Section \ref{Background Works} reviews the background work. Section \ref{LSTMFCN} presents the architecture of the proposed models. Section \ref{Experiments} analyzes and discusses theour experiments performed. Finally, we draw conclusions are drawn in Section \ref{conclusion}. 



==> literature_review.tex <==
\subsection{Temporal Convolutions}
The input to a Temporal Convolutional Network is generally a time series signal. As stated in \textit{Lea et al.}\cite{Lea_2016}, let $X_{t} \in \mathbb{R}^{F_0}$ be the input feature vector of length $F_0$ for time step $t$ for $0 < t \leq T$. Note that the time T may vary for each sequence, and we denote the number of time steps in each layer as $T_l$. The true action label for each frame is given by $y_t \in \{1, . . . , C\}$, where C is the number of classes.

Consider $L$ convolutional layers. We apply a set of 1D filters on each of these layers that capture how the input signals evolve over the course of an action. According to \textit{Lea et al.} \cite{Lea_2016}, the filters for each layer are parameterized by tensor $W^{(l)} \in \mathbb{R}^{F_l \times d \times F_{l-1}} $ and biases $b^{(l)} \in \mathbb{R}^{F_l}$, where $l \in \{1, . . . , L\}$ is the layer index and $d$ is the filter duration. For the $l$-th layer, the $i$-th component of the (unnormalized) activation ${\mathbf {\hat{E}}}^{(l)}_{t} \in \mathbb{R}^{F_{l}}$ is a function of the incoming (normalized) activation matrix $E^{(l-1)} \in \mathbb{R}^{F_{l-1} \times T_{l-1}}$ from the previous layer 
\begin{equation}
{\mathbf {\hat{E}}}_{i, t}^{(l)} = f\left(b_{i}^{(l)} + \sum_{t'=1}^{d} \left< W_{i, t', .}^{(l)}, E_{., t+d-t'}^{(l-1)} \right> \right)
\end{equation}
for each time $t$ where $f(\cdot)$ is a Rectified Linear Unit.

We use Temporal Convolutional Networks as a feature extraction module in a Fully Convolutional Network (FCN) branch. A basic convolution block consists of a convolution layer, followed by batch normalization \cite{ioffe2015batch}, followed by an activation function, which can be either a Rectified Linear Unit or a Parametric Rectified Linear Unit \cite{Trottier2016}.

\subsection{Recurrent Neural Networks}
\def\x{{\mathbf x}}
\def\L{{\cal L}}
Recurrent Neural Networks, often shortened to RNNs, are a class of neural networks which exhibit temporal behaviour due to directed connections between units of an individual layer. As reported by \textit{Pascanu et al.} \cite{pascanu2013construct}, recurrent neural networks maintain a hidden vector $\mathbf h$, which is updated at time step $t$ as follows:
 
\begin{equation}
	\mathbf h_t = \tanh(\mathbf W\mathbf h_{t-1} + \mathbf I\mathbf  \x_t),
\end{equation}
tanh is the hyperbolic tangent function, $\mathbf W$ is the recurrent weight matrix and $\mathbf I$ is a projection matrix. The hidden state $\mathbf h$ is  used to make a prediction

\begin{equation}
	\mathbf y_t = \text{softmax}(\mathbf W\mathbf h_{t-1}),
\end{equation}
softmax provides a normalized probability distribution over the possible classes, $\sigma$ is the logistic sigmoid function and $\mathbf W$ is a weight matrix. By using $\mathbf h$ as the input to another RNN, we can stack RNNs, creating deeper architectures 

\begin{equation}
	\mathbf h_t^{l} = \sigma(\mathbf W\mathbf h_{t-1}^{l} + \mathbf I\mathbf h_t^{l-1}).
\end{equation}

\subsection{Long Short-Term Memory RNNs}
\def\x{{\mathbf x}}

Long short-term memory recurrent neural networks are an improvement over the general recurrent neural networks, which possess a vanishing gradient problem. As stated in \textit{Hochreiter et al.}\cite{hochreiter1997long}, LSTM RNNs address the vanishing gradient problem commonly found in ordinary recurrent neural networks by incorporating gating functions into their state dynamics. At each time step, an LSTM maintains a hidden vector $\mathbf h$ and a memory vector $\mathbf m$  responsible for controlling state updates and outputs. More concretely, \textit{Graves et al.} \cite{graves2012supervised} define the computation at time step $t$ as follows :
\begin{equation}
	\begin{split}
		& \mathbf g^u = \sigma(\mathbf W^u\mathbf h_{t-1}  + \mathbf I^u\x_t ) \\
		& \mathbf g^f = \sigma(\mathbf W^f\mathbf h_{t-1} + \mathbf I^f\x_t) \\
		& \mathbf g^o = \sigma(\mathbf W^o\mathbf h_{t-1} + \mathbf I^o\x_t) \\
		& \mathbf g^c = \tanh(\mathbf W^c\mathbf h_{t-1} + \mathbf I^c\x_t) \\
		& \mathbf m_t = \mathbf g^f \odot \mathbf m_{t-1}\mathbf \ + \  \mathbf g^u \odot 
		\mathbf g^c \\
		& \mathbf h_t = \tanh(\mathbf g^o \odot \mathbf m_t) 
	\end{split}
\end{equation}
where $\sigma$ is the logistic sigmoid function, $\odot$ represents elementwise multiplication, $\mathbf W^u, \mathbf W^f, \mathbf W^o, \mathbf W^c$ are recurrent weight matrices and $\mathbf I^u, \mathbf I^f, \mathbf I^o, \mathbf I^c$ are projection matrices.

While LSTMs possess the ability to learn temporal dependencies in sequences, they have difficulty with long term dependencies in long sequences. The attention mechanism proposed by \textit{Bahdanau et al.} \cite{bahdanau2014neural} can help the LSTM RNN learn these dependencies. %Bi-directional LSTMs \cite{schuster1997bidirectional}, which read the input sequence in both forward and backward directions, are able to learn these long term dependencies.

\subsection{Attention Mechanism}
The attention mechanism is a technique often used in neural translation of text, where a context vector $C$ is conditioned on the target sequence $y$. As discussed in \textit{Bahdanau et al.}\cite{bahdanau2014neural}, the context vector $c_i$ depends on a sequence of \textit{annotations} $(h_1, ..., h_{T_{x}})$ to which an encoder maps the input sequence. Each annotation $h_i$ contains information about the whole input sequence with a strong focus on the parts surrounding the $i$-th word of the input sequence.

The context vector $c_i$ is then computed as a weighted sum of these annotations $h_i$:
\begin{equation}
    c_i = \sum_{j=1}^{T_x} \alpha_{ij}h_j.
\end{equation}

The weight $\alpha_{ij}$ of each annotation $h_j$ is computed by : 
\begin{equation}
    \alpha_{ij} = \frac{exp(e_{ij})}{\sum_{k=1}^{T_x} exp(e_{ik})}
\end{equation}
where $e_{ij} = a(s_{i-1}, h_j)$ is an \textit{alignment model}, which scores how well the input around position $j$ and the output at position $i$ match. The score is based on the RNN hidden state $s_{i−1}$ and the $j$-th annotation $h_j$ of the input sentence. 


\begin{figure*}
\center
\fbox{
\includegraphics[width=0.75\linewidth]{"with_attention".pdf}
}
\center
\caption{The LSTM-FCN architecture. LSTM cells can be replaced by Attention LSTM cells to construct the ALSTM-FCN architecture.}
\label{fig:arch}

\end{figure*}

\textit{Bahdanau et al.}\cite{bahdanau2014neural} parametrize the alignment model $a$ as a feedforward neural network which is jointly trained with all the other components of the model. The alignment model directly computes a soft alignment, which allows the gradient of the cost function to be backpropagated. %According to \textit{Bahdanau et al.}\cite{bahdanau2014neural}, this gradient can be used to train the alignment model as well as the whole translation model jointly.
